Training with Mixed-Precision Floating-Point Assignments

When training deep neural networks, keeping all tensors in high precision (e.g., 32-bit or even 16-bit floats) is often wasteful. However, keeping all tensors in low precision (e.g., 8-bit floats) can lead to unacceptable accuracy loss. Hence, it is important to use a precision assignment -- a mapping from all tensors (arising in training) to precision levels (high or low) -- that keeps most of the tensors in low precision and leads to sufficiently accurate models. We provide a technique that explores this memory-accuracy tradeoff by generating precision assignments for convolutional neural networks that (i) use less memory and (ii) lead to more accurate convolutional networks at the same time, compared to the precision assignments considered by prior work in low-precision floating-point training. We evaluate our technique on image classification tasks by training convolutional networks on CIFAR-10, CIFAR-100, and ImageNet. Our method typically provides > 2x memory reduction over a baseline precision assignment while preserving training accuracy, and gives further reductions by trading off accuracy. Compared to other baselines which sometimes cause training to diverge, our method provides similar or better memory reduction while avoiding divergence.

==> paper/_paper-mlsys.tex <==
%%%%%%%% mlsys 2022 EXAMPLE LATEX SUBMISSION FILE %%%%%%%%%%%%%%%%%

%% \documentclass{article}

% Recommended, but optional, packages for figures and better typesetting:
\usepackage{microtype}
\usepackage{graphicx}
%\usepackage{subfigure} %% WL: not compatible with subcaption.
\usepackage{booktabs} % for professional tables

% hyperref makes hyperlinks in the resulting PDF.
% If your build breaks (sometimes temporarily if a hyperlink spans a page)
% please comment out the following usepackage line and replace
% \usepackage{mlsys2023} with \usepackage[nohyperref]{mlsys2023} above.
\usepackage{hyperref}

% Attempt to make hyperref and algorithmic work together better:
\newcommand{\theHalgorithm}{\arabic{algorithm}}

% % Use the following line for the initial blind version submitted for review:
% \usepackage{paper/mlsys2023}
% If accepted, instead use the following line for the camera-ready submission:
% \usepackage[accepted]{mlsys2023}
%%%%%%%%%%%%%%%%%%%%
% preprint option (added by WL)
\usepackage[preprint]{paper/mlsys2023}
%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
%\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
%\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
%\usepackage{microtype}      % microtypography
%\usepackage{xcolor}         % colors
\usepackage{natbib}  %% WL: [numbers, sort&compress] ?
\usepackage[all=normal,paragraphs]{savetrees}
\input{paper/macro}

%%% multibib
\newcites{A}{References (for Appendix)}
%%%%%%%%%%%%%%%%%%%%


% The \mlsystitle you define below is probably too long as a header.
% Therefore, a short form for the running title is supplied here:
\mlsystitlerunning{Training with Mixed-Precision Floating-Point Assignments}
%\mlsystitlerunning{Exploring Memory-Accuracy Tradeoff in Training via Mixed-Precision Floating-Point Assignment}
%% Low-Precision Floating-Point Training: Memory-Accuracy Trade-Off via Per-Tensor Precision
%% Low-Precision Floating-Point Training with Per-Tensor Precision

\begin{document}

\twocolumn[
\mlsystitle{Training with Mixed-Precision Floating-Point Assignments}
%\mlsystitle{Exploring Memory-Accuracy Tradeoff in Training \\ via Mixed-Precision Floating-Point Assignments}

% It is OKAY to include author information, even for blind
% submissions: the style file will automatically remove it for you
% unless you've provided the [accepted] option to the mlsys2023
% package.

% List of affiliations: The first argument should be a (short)
% identifier you will use later to specify author affiliations
% Academic affiliations should list Department, University, City, Region, Country
% Industry affiliations should list Company, City, Region, Country

% % You can specify symbols, otherwise they are numbered in order.
% % Ideally, you should not use this facility. Affiliations will be numbered
% % in order of appearance and this is the preferred way.
% \mlsyssetsymbol{equal}{*}

\begin{mlsysauthorlist}
\mlsysauthor{Wonyeol Lee}{stanford}
\mlsysauthor{Rahul Sharma}{msr}
\mlsysauthor{Alex Aiken}{stanford}
\end{mlsysauthorlist}

\mlsysaffiliation{stanford}{Stanford University, USA}
\mlsysaffiliation{msr}{Microsoft Research, India}

\mlsyscorrespondingauthor{Wonyeol Lee}{wonyeol.lee.cs@gmail.com}
% \mlsyscorrespondingauthor{Rahul Sharma}{rahsha@microsoft.edu}
% \mlsyscorrespondingauthor{Alex Aiken}{aaiken@stanford.edu}

% % You may provide any keywords that you
% % find helpful for describing your paper; these are used to populate
% % the "keywords" metadata in the PDF but will not be shown in the document
% \mlsyskeywords{Machine Learning, MLSys}

\vskip 0.3in

\input{paper/0-abstr}
]

% this must go after the closing bracket ] following \twocolumn[ ...

% This command actually creates the footnote in the first column
% listing the affiliations and the copyright notice.
% The command takes one argument, which is text to display at the start of the footnote.
% The \mlsysEqualContribution command is standard text for equal contribution.
% Remove it (just {}) if you do not need this facility.

\printAffiliationsAndNotice{}  % leave blank if no need to mention equal contribution
% \printAffiliationsAndNotice{\mlsysEqualContribution} % otherwise use the standard text.


%%%%%%%%%%%%%%%%%%%%
\input{paper/1-intro}
\input{paper/2-related}
\input{paper/3-prob}
\input{paper/4-algo}
\input{paper/5-eval}
\input{paper/6-concl}
%\input{paper/7-ack}

%\bibliographystyle{paper/abbrvnatnew}
\bibliographystyle{paper/mlsys2023}
\bibliography{paper/ref}

\appendix
\input{paper/8-appdx-prob}
\input{paper/8-appdx-eval}
\clearpage
% \bibliographystyleA{paper/abbrvnatnew}
\bibliographystyleA{paper/mlsys2023}
\bibliographyA{paper/ref}

% \clearpage
% \input{paper/3-algo-v1}
%%%%%%%%%%%%%%%%%%%%


\end{document}

